Dynamic DBSCAN with Euler Tour Sequences

We propose a fast and dynamic algorithm for Density-Based Spatial Clustering of Applications with Noise (DBSCAN) that efficiently supports online updates. Traditional DBSCAN algorithms, designed for batch processing, become computationally expensive when applied to dynamic datasets, particularly in large-scale applications where data continuously evolves. To address this challenge, our algorithm leverages the Euler Tour Trees data structure, enabling dynamic clustering updates without the need to reprocess the entire dataset. This approach preserves a near-optimal accuracy in density estimation, as achieved by the state-of-the-art static DBSCAN method (Esfandiari et al., 2021) Our method achieves an improved time complexity of $O(d \log^3(n) + \log^4(n))$ for every data point insertion and deletion, where $n$ and $d$ denote the total number of updates and the data dimension, respectively. Empirical studies also demonstrate significant speedups over conventional DBSCANs in real-time clustering of dynamic datasets, while maintaining comparable or superior clustering quality.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne '') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}

==> notation.tex <==
% Apply this command to all notation
% \newcommand{\allnotation}[1]{\textcolor{red}{#1}}
\newcommand{\allnotation}[1]{#1}

% Start with 'theorem' like commands.
% \newtheorem{theorem}{Theorem} [chapter]
\newtheorem{conjecture}{Conjecture} [section]
\newtheorem{lemma}{Lemma} [section]
\newtheorem{remark}{Remark} [section]
\newtheorem{definition}{Definition} [section]
\newtheorem{corollary}{Corollary} [section]
\newtheorem{proposition}{Proposition} [section]
\newtheorem{example}{Example} [section]
\newtheorem{openquestion}{Open Question}
\newtheorem{mainresult}{Main Result}

% Add various mathematical commands
\newcommand{\transpose}{\intercal}                    % Transpose
\newcommand{\conjtranspose}{\dagger}                  % Conjugate transpose
\newcommand{\inner}[2]{\left\langle #1 , #2 \right\rangle} % <a,b>
\newcommand{\norm}[1]{\left\| #1\right\|}                  % ||a||
\newcommand{\abs}[1]{\left\lvert#1\right\rvert}
\DeclareMathOperator*{\argmin}{arg\,min}        % arg min
\DeclareMathOperator*{\argmax}{arg\,max}        % arg max
\newcommand{\tr}{\mathrm{tr}}                   % trace
\newcommand{\calL}{\mathcal{L}}
\newcommand{\supp}{\mathrm{supp}}
\newcommand{\sign}{\mathrm{sign}}
\newcommand{\poly}{\mathrm{poly}}
\renewcommand{\P}{\mathsf{P}}
\newcommand{\NP}{\mathsf{NP}}

% We will add latex commands for all of our notation conventions.
\renewcommand{\vec}[1]{{\allnotation{\bm{#1}}}}
\newcommand{\vecf}{\vec{f}}
\newcommand{\vecg}{\vec{g}}
\newcommand{\vecx}{\vec{x}}
\newcommand{\vecy}{\vec{y}}
\newcommand{\vecz}{\vec{z}}
\newcommand{\vecu}{\vec{u}}
\newcommand{\vecv}{\vec{v}}
\newcommand{\vecr}{\vec{r}}
\newcommand{\vecp}{\vec{p}}
\newcommand{\vecs}{\vec{s}}
\newcommand{\veca}{\vec{a}}
\newcommand{\vecb}{\vec{b}}
\newcommand{\vecw}{\vec{w}}
\newcommand{\vecc}{\vec{c}}
\newcommand{\constvec}{\vec{1}}
\newcommand{\zerovec}{\vec{0}}
\newcommand{\indicatorvec}{\vec{\chi}}
\newcommand{\statdist}{\vec{\pi}}

\newcommand{\graph}[1]{{\allnotation{#1}}}
\newcommand{\graphg}{\graph{G}}
\newcommand{\graphh}{\graph{H}}
\newcommand{\graphm}{\graph{M}}

\newcommand{\set}[1]{{\allnotation{#1}}}
\newcommand{\setv}{\set{V}}
\newcommand{\sete}{\set{E}}
\newcommand{\sets}{\set{S}}
\newcommand{\sett}{\set{T}}
\newcommand{\setl}{\set{L}}
\newcommand{\setr}{\set{R}}
\newcommand{\seta}{\set{A}}
\newcommand{\setb}{\set{B}}
\newcommand{\setc}{\set{C}}
\newcommand{\setu}{\set{U}}
\newcommand{\setp}{\set{P}}
\newcommand{\setm}{\set{M}}
\newcommand{\vertexset}{\setv}
\newcommand{\vertexsetg}{\vertexset_\graphg}
\newcommand{\vertexseth}{\vertexset_\graphh}
\newcommand{\edgeset}{\sete}
\newcommand{\edgesetg}{\edgeset_\graphg}
\newcommand{\edgeseth}{\edgeset_\graphh}

\newcommand{\mat}[1]{{\allnotation{\mathbf{#1}}}}
\newcommand{\mata}{\mat{A}}
\newcommand{\matb}{\mat{B}}
\newcommand{\matm}{\mat{M}}

% Graph matrices
\newcommand{\lap}{\mat{L}}
\newcommand{\lapn}{\mat{N}}
\newcommand{\signlap}{\mat{J}}
\newcommand{\signlapn}{\mat{Z}}
\newcommand{\degm}{\mat{D}}
\newcommand{\degmhalf}{\degm^{\allnotation{\frac{1}{2}}}}
\newcommand{\degmhalfneg}{\degm^{\allnotation{-\frac{1}{2}}}}
\newcommand{\adj}{\mat{A}}
\newcommand{\adjn}{\mat{B}}
\newcommand{\adjh}{\allnotation{\mat{A}_h}}
\newcommand{\lazywalkm}{\mat{W}}
\newcommand{\walkm}{\mat{X}}

% Other matrices
\newcommand{\identity}{\mat{I}}

% Other maths
\newcommand{\imag}{\allnotation{\mathit{i}}}
\newcommand{\conjugate}[1]{\allnotation{\overline{#1}}}

% Just always use varepsilon
\renewcommand{\epsilon}{\varepsilon}

% Commands for consistent formatting of certain words
\newcommand{\pagerank}{Pagerank}
\newcommand{\lovasz}{Lov\'asz}
\newcommand{\etal}{et al.}

% How should we represent the QED symbol throughout the thesis?
\renewcommand\qedsymbol{$\blacksquare$}

% Graph theory
\renewcommand{\deg}{{\allnotation{d}}}
\newcommand{\weight}{{\allnotation{w}}}
\newcommand{\bipart}{{\allnotation{\beta}}}
\newcommand{\cond}{{\allnotation{\Phi}}}
\newcommand{\kcond}{{\allnotation{\rho}}}
\newcommand{\kcondg}{{\allnotation{\kcond_\graphg}}}
\newcommand{\cutimb}{{\allnotation{\mathrm{CI}}}} % Cut Imbalance
\newcommand{\neighbors}{{\allnotation{N}}}
\newcommand{\connected}{{\allnotation{\sim}}}
\newcommand{\boundary}{{\allnotation{\partial}}}
\newcommand{\vol}{\mathrm{vol}}

% Pagerank
\newcommand{\ppr}{\mathrm{ppr}}
\newcommand{\apr}{\mathrm{apr}}

% Diffusion process
\newcommand{\discrep}{{\allnotation{\Delta}}}

% First definition
\newcommand{\firstdef}[1]{\textbf{#1}}

% Iverson Bracket
\newcommand{\iverson}[1]{\pmb{\left[\vphantom{#1}\right.} #1 \pmb{\left.\vphantom{#1}\right]}}

% Complexity
\newcommand{\bigo}[1]{O\!\left(#1\right)}
\newcommand{\bigomega}[1]{\Omega\!\left(#1\right)}
\newcommand{\bigtheta}[1]{\Theta\!\left(#1\right)}
\newcommand{\bigotilde}[1]{\widetilde{O}\!\left(#1\right)}
\newcommand{\polylog}{\mathrm{polylog}}
\newcommand{\opt}{\mathrm{OPT}}

% Probability
\newcommand{\E}{\mathbb{E}}
\newcommand{\p}{\mathbb{P}}
\newcommand{\expected}[1]{\E\left[#1\right]}
\newcommand{\prob}[1]{\p\left[#1\right]}
\newcommand{\I}{\mathbb{I}}

% Sets
\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\union}{\cup}
\newcommand{\intersect}{\cap}
\newcommand{\cardinality}[1]{\abs{#1}}
\newcommand{\setcomplement}[1]{\overline{#1}}
\newcommand{\comp}[1]{\overline{#1}}
\newcommand{\symmetricdiff}{\triangle}

% Colored text
\newcommand{\todo}[1]{\textcolor{red}{\textbf{ToDo:} #1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\green}[1]{\textcolor{green}{#1}}

% Multi part definitions
\newcommand{\twopartdef}[4]
{
	\left\{
		\begin{array}{ll}
			#1 & \mbox{if } #2 \\
			#3 & \mbox{if } #4
		\end{array}
	\right.
}

\newcommand{\twopartdefow}[3]
{
	\left\{
		\begin{array}{ll}
			#1 & \mbox{if } #2 \\
			#3 & \mbox{otherwise}
		\end{array}
	\right.
}

\newcommand{\twopartdefowfs}[3]
{
	\left\{
		\begin{array}{ll}
			#1 & \mbox{if } #2, \\
			#3 & \mbox{otherwise.}
		\end{array}
	\right.
}

\newcommand{\threepartdef}[6]
{
	\left\{
		\begin{array}{lll}
			#1 & \mbox{if } #2 \\
			#3 & \mbox{if } #4 \\
			#5 & \mbox{if } #6
		\end{array}
	\right.
}

\newcommand{\threepartdefow}[5]
{
	\left\{
		\begin{array}{lll}
			#1 & \mbox{if } #2 \\
			#3 & \mbox{if } #4 \\
			#5 & \mbox{otherwise}
		\end{array}
	\right.
}

% Bibliography helper functions
\newcommand{\FOCS}[2]{#1 Annual IEEE Symposium on Foundations of Computer Science
(FOCS'#2)}
\newcommand{\STOC}[2]{#1 Annual ACM Symposium on Theory of Computing (STOC'#2)}
\newcommand{\SODA}[2]{#1 Annual ACM-SIAM Symposium on Discrete Algorithms (SODA'#2)}
\newcommand{\ICALP}[2]{#1 International Colloquium on Automata, Languages, and Programming (ICALP'#2)}
\newcommand{\PODC}[2]{#1 Annual ACM-SIGOPT Principles of Distributed Computing
(PODS'#2)}
\newcommand{\STACS}[2]{#1 International Symposium on Theoretical Aspects of Computer
Science (STACS'#2)}
\newcommand{\ISAAC}[2]{#1 International Symposium on Algorithms and Computation
(ISAAC'#2)}
\newcommand{\WG}[2]{#1 Workshop of Graph-Theoretic Concepts in Computer Science
(WG'#2)}
\newcommand{\NIPS}[2]{#1 Advances in Neural Information Processing Systems
(NeurIPS'#2)}
\newcommand{\RANDOM}[2]{#1 International Workshop on Randomization and Computation
(RANDOM'#2)}
\newcommand{\CCC}[2]{#1 Conference on Computational Complexity
(CCC'#2)}
\newcommand{\ICML}[2]{#1 International Conference on Machine Learning
(ICML'#2)}
\newcommand{\ICLR}[2]{#1 International Conference on Learning Representations 
(ICLR'#2)}
\newcommand{\ICDM}[2]{#1 International Conference on Data Mining 
(ICDM'#2)}
\newcommand{\AISTATS}[2]{#1 International Conference on
Artificial Intelligence and Statistics (AISTATS'#2)}
\newcommand{\ITCS}[2]{#1 Innovations in Theoretical Computer Science (ITCS'#2)}
\newcommand{\SPAA}[2]{#1 ACM Symposium on Parallelism in Algorithms and Architectures (SPAA'#2)}
\newcommand{\KDD}[2]{#1 ACM SIGKDD International Conference on Knowledge Discovery and Data Mining (KDD'#2)}

==> sections_aistats/related.tex <==
\section{Related Work}\label{sec:related}
\begin{itemize}
    \item Cite DBSCAN results
    \item maybe other dynamic clustering results
    \item Dynamic Trees
\end{itemize}
